Learning Semantics for Visual Place Recognition through Multi-Scale Attention

In this paper we address the task of visual place recognition (VPR), where the goal is to retrieve the correct GPS coordinates of a given query image against a huge geotagged gallery. While recent works have shown that building descriptors incorporating semantic and appearance information is beneficial, current state-of-the-art methods opt for a top down definition of the significant semantic content. Here we present the first VPR algorithm that learns robust global embeddings from both visual appearance and semantic content of the data, with the segmentation process being dynamically guided by the recognition of places through a multi-scale attention module. Experiments on various scenarios validate this new approach and demonstrate its performance against state-of-the-art methods. Finally, we propose the first synthetic-world dataset suited for both place recognition and segmentation tasks.

==> Images/pooling.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Images/imgs/ch3_pooling_v2.pdf}
    \vspace{2pt}
    \caption{Illustration of the multi-scale pooling module. Different from prior works, features extracted at different levels of the shared encoder are exploited to compute the global descriptors. $\otimes$ indicates up-sampling and channel-wise dot product. $\oplus$ indicates channel-wise concatenation.}
    \label{fig:pooling}
    \vspace{-6pt}
\end{figure}

==> Sections/6_Ablation.tex <==
\section{Ablation study}
\noindent
We performed an extensive ablation study on the RobotCar \cite{Maddern_IJRR2017} scenarios
to evaluate the impact of each component of our method. For this study we used ResNet50 as encoder and DeepLabv2  \cite{Chen2018DeepLabSI} as SemSeg decoder.
As baseline, we consider the shared encoder followed by the GeM \cite{Radenovic_PAMI2019} pooling layer. Then, we added each component, \ie, the multi-scale attention block (Att), the segmentation decoder (SemSeg), the attention to guide the segmentation (G-SemSeg) and the unsupervised domain adaptation mechanism (DA), trying all combinations. 
As shown in \cref{tab:ablation} each module improves the results, in particular across the single-scale embedding experiments even without the domain adaptation (DA) task, the semantic segmentation (SemSeg) and the guided configuration (G-SemSeg) provide strong boosts respectively of +10\% and +14\% on the average. 
Finally, we build the final architecture that adds up to an overall improvement of approximately 17\% over the baseline. 
Moreover, adding our novel multi-scale embeddings (ms-GeM) gives a further gain of 4\%. Due to the lack of space, we include an extended version of \cref{tab:ablation} in the supplementary material. 



==> Tables/ablation.tex <==
% tabella ablation
\begin{table*}[ht]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{ccccccccc|c|c}
\hline
\begin{tabular}[c]{@{}c@{}}ms-GeM\end{tabular} & 
\begin{tabular}[c]{@{}c@{}} Att\end{tabular} & 
SemSeg &
\begin{tabular}[c]{@{}c@{}} G-SemSeg\end{tabular} &
DA &
\begin{tabular}[c]{@{}c@{}}Overcast/Rain\\ 1 / 5 / 10\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Overcast/Snow\\ 1 / 5 / 10\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Overcast/Sun\\ 1 / 5 / 10\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Overcast/Night\\ 1 / 5 / 10\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Avg\\ 1 / 5 / 10\end{tabular} &
Avg \\ 
\hline
 &   &   &   &   & 71.4 / 83.8 / 87.9 & 37.6 / 55.1 / 63.6 & 30.9 / 47.9 / 55.7 & 4.4 / 12.2 / 18.3 & 36.1 / 49.7 / 56.4 & 47.4 \\
 & $\checkmark$ &   &   &   & 71.4 / 83.7 / 88.0 & 40.6 / 59.3 / 67.2 & 31.1 / 50.3 / 59.1 & 4.9 / 15.1 / 21.9 & 37.0 / 52.1 / 59.1 & 49.4 \\
 & $\checkmark$ & $\checkmark$ &   &   & 82.7 / 93.3 / 95.5 & 50.0 / 70.1 / 79.2 & 45.5 / 66.2 / 74.4 & 7.5 / 17.9 / 25.9 & 46.4 / 61.9 / 68.8 & 59.0 \\
 & $\checkmark$ & & & $\checkmark$ & 86.8 / 93.8 / 96.2 & 56.1 / 73.6 / 80.6 & 43.8 / 64.0 / 72.6 & 6.5 / 16.9 / 25.4 & 48.3 / 62.1 / 68.7 & 59.7 \\ 
 & $\checkmark$ & $\checkmark$ &   & $\checkmark$ & 81.4 / 92.3 / 94.8 & 53.6 / 73.3 / 81.3 & 44.1 / 64.6 / 72.9 & 10.2 / 24.6 / 34.7 & 47.3 / 63.7 / 70.9 & 60.6 \\
 & $\checkmark$ & $\checkmark$ & $\checkmark$ &   & 87.6 / 95.1 / 96.7 & 56.3 / 75.7 / 83.0 & 50.3 / 69.6 / 84.1 & 8.8 / 20.2 / 29.2 & 50.8 / 65.1 / 73.3 & 63.1 \\
 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 85.2 / 94.1 / 96.3 & 59.5 / 78.7 / 85.3 & 50.5 / 69.1 / 76.9 & \textbf{11.7 / 27.2 / 37.3} & 51.7 / 67.3 / 73.9 & 64.3 \\
 \hline
$\checkmark$ &   &   &   &   & 85.8 / 93.4 / 95.6 & 56.5 / 72.6 / 79.1 & 51.0 / 69.5 / 76.6 & 7.4 / 20.0 / 29.2 & 50.2 / 63.9 / 70.1 & 61.4 \\
$\checkmark$ & $\checkmark$ &   &   &   & 90.5 / 96.3 / 97.5 & 59.2 / 75.9 / 82.6 & 50.1 / 67.8 / 75.2 & 5.8 / 16.4 / 25.7 & 51.4 / 64.1 / 70.3 & 61.9 \\
$\checkmark$ & $\checkmark$ & $\checkmark$ &   &   & 91.1 / 96.0 / 97.0 & 55.6 / 72.7 / 79.5 & 54.8 / 72.2 / 79.2 & 7.1 / 17.4 / 25.5 & 52.2 / 64.6 / 70.3 & 62.4 \\
$\checkmark$ & $\checkmark$ & & & $\checkmark$ & 87.6 / 94.8 / 96.6 & 60.3 / 78.0 / 84.1 & 48.9 / 68.7 / 75.7 & 7.9 / 20.2 / 29.0 & 51.2 / 65.4 / 71.3 & 62.6 \\
$\checkmark$ & $\checkmark$ & $\checkmark$ &   & $\checkmark$ & 89.9 / 96.0 / 97.3 & 63.1 / 80.4 / 86.4 & 57.9 / 75.6 / 81.6 & 7.7 / 18.6 / 27.7 & 54.6 / 67.6 / 73.3 & 65.2 \\
$\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ &   & 91.5 / 96.4 / 97.3 & 58.4 / 74.6 / 80.6 & 53.9 / 72.2 / 78.9 & 7.9 / 20.8 / 29.8 & 53.0 / 66.0 / 71.7 & 63.5 \\
$\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & \textbf{92.2 / 96.8 / 97.8} & \textbf{68.0 / 83.4 / 89.0} & \textbf{62.6 / 79.6 / 85.0} & 11.3 / 24.5 / 34.1 & \textbf{58.5 / 71.1 / 76.5} & \textbf{68.7} \\ 
\hline
\end{tabular}
\end{adjustbox}
\vspace{2pt}
\caption{Ablation study to assess the contribution of each component in our architecture. \emph{ms-GeM} stays for Multi-Scale Embeddings obtained through our new multi-scale pooling layer, \emph{Att} indicates that the attention module is used in the VPR task, \emph{SemSeg} and \emph{G-SemSeg} denote that Semantic Segmentation and Guided Semantic Segmentation are active, while \emph{DA} stands for the Domain Adaptation task.}
\label{tab:ablation}
\end{table*}


==> Tables/num_images.tex <==
% table: dataset details
\begin{table}[t!]
\centering
\begin{adjustbox}{width=0.6\textwidth}

 \begin{tabular}{l|l|l|l}
        Specs                   & Virtual KITTI 2   & SYNTHIA       & \textbf{Ours}         \\ 
        \hline
        Size                    & 21359             & 200000        & 43604                 \\
        \#imgs per scene        & 447               & 8000          & 10091                 \\
        Classes                 & 16                & 13            & 25                    \\
        Gallery/Query           & \xmark            & \xmark        & \cmark                \\                 
        GPS/IMU                 & \xmark            & \xmark        & \cmark                \\
        \end{tabular}

\end{adjustbox}
\vspace{2pt}
\caption{Comparison between our dataset, Virtual KITTI 2 and the SYNTHIA synthetic datasets.}
\label{tab:whole_idda}
\vspace{-6pt}
\end{table}










\begin{comment}
\begin{table}[t!]
\begin{adjustbox}{width=\columnwidth}
\centering
\begin{tabular}{l|l|l}
Specs                                                                     & Virtual KITTI 2                                                                                   & \textbf{Ours}                                                                  \\ 
\hline\hline
\begin{tabular}[c]{@{}l@{}}\\Dimension \end{tabular}                      & \begin{tabular}[c]{@{}l@{}}\\21359 \end{tabular}                                                  & \begin{tabular}[c]{@{}l@{}}\\43604 \end{tabular}                               \\ 
\hline
\begin{tabular}[c]{@{}l@{}}\\Views \end{tabular}                          & \begin{tabular}[c]{@{}l@{}}5 (front, 15\degree left,~15\degree right, \\30\degree left, 30\degree right) \end{tabular}          & \begin{tabular}[c]{@{}l@{}}4 (front, rear, \\ left, right) \end{tabular}       \\ 
\hline
\begin{tabular}[c]{@{}l@{}}\\Environment \end{tabular}                    & \begin{tabular}[c]{@{}l@{}}Mixed image of mid-size city,\\ rural areas and highways \end{tabular} & \begin{tabular}[c]{@{}l@{}}2 urban cities (Town03\\ and Town10) \end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}\\Weather Condition \end{tabular}              & \begin{tabular}[c]{@{}l@{}}Fog, Morning, Overcast, \\ Rain, Sunset \end{tabular}                  & \begin{tabular}[c]{@{}l@{}}Clear Noon, Hard Rain \\ Sunset \end{tabular}       \\ 
\hline
\begin{tabular}[c]{@{}l@{}}\# Images \\ (avg. per scenario) \end{tabular} & \begin{tabular}[c]{@{}l@{}}\\447 \end{tabular}                                                    & \begin{tabular}[c]{@{}l@{}}\\10091 \end{tabular}                               \\ 
\hline
\begin{tabular}[c]{@{}l@{}}\\Semantic Classes \end{tabular}               & \begin{tabular}[c]{@{}l@{}}\\16 \end{tabular}                                                     & \begin{tabular}[c]{@{}l@{}}\\25 \end{tabular}                                  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}\\Gallery, Query\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}\\\xmark\end{tabular}                                   & \begin{tabular}[c]{@{}l@{}}\\\cmark\end{tabular}                \\ 
\hline
\begin{tabular}[c]{@{}l@{}}\\GPS/IMU \end{tabular}                        & \begin{tabular}[c]{@{}l@{}}\\\xmark\end{tabular}                                   & \begin{tabular}[c]{@{}l@{}}\\\cmark\end{tabular}               
\end{tabular}
\end{adjustbox}
\vspace{2pt}
\caption{Comparison between our dataset and the Virtual KITTI 2 synthetic dataset.}
\label{tab:whole_idda}
\end{table}
\end{comment}
